A Multi-Grained Self-Interpretable Symbolic-Neural Model For Single/Multi-Labeled Text Classification

Deep neural networks based on layer-stacking architectures have historically suffered from poor inherent interpretability. Meanwhile, symbolic probabilistic models function with clear interpretability, but how to combine them with neural networks to enhance their performance remains to be explored. In this paper, we try to marry these two systems for text classification via a structured language model. We propose a Symbolic-Neural model that can learn to explicitly predict class labels of text spans from a constituency tree without requiring any access to span-level gold labels. As the structured language model learns to predict constituency trees in a self-supervised manner, only raw texts and sentence-level labels are required as training data, which makes it essentially a general constituent-level self-interpretable classification model. Our experiments demonstrate that our approach could achieve good prediction accuracy in downstream tasks. Meanwhile, the predicted span labels are consistent with human rationales to a certain degree.

==> related_works.tex <==
\section{Related works}
\vspace{-5pt}
\paragraph{Structured language models.} Many attempts have been made to develop structured language models. \cite{DBLP:journals/ai/Pollack90} proposed to use RvNN as a recursive architecture to encode text hierarchically, and \cite{DBLP:conf/emnlp/SocherPWCMNP13} showed the effectiveness of RvNNs with gold trees for sentiment analysis. However, both approaches require annotated trees. Gumbel-Tree-LSTMs~\citep{DBLP:conf/aaai/ChoiYL18} construct trees by recursively selecting two terminal nodes to merge and learning composition probabilities via downstream tasks. CRvNN~\citep{DBLP:conf/icml/ChowdhuryC21} makes the entire process end-to-end differentiable and parallel by introducing a continuous relaxation. However, neither Gumbel-Tree-LSTMs nor CRvNN mention the pretraining mechanism in their work. URNNG~\citep{dblp:conf/naacl/kimrykdm19} proposed the first architecture to jointly pretrain a parser and an encoder based on RNNG \citep{dyer-etal-2016-recurrent}. However, its $O(n^3)$ time and space complexity makes it hard to pretrain on large-scale corpora. 
ON-LSTM and StructFormer~\citep{DBLP:conf/iclr/ShenTSC19,DBLP:conf/acl/ShenTZBMC20} propose a series of methods to integrate structures into LSTM or Transformer by masking information in differentiable ways. As the encoding process is still performed in layer-stacking models, there are no intermediate representations for tree nodes. \cite{DBLP:journals/corr/MaillardCY17} propose an alternative approach, based on a differentiable CKY encoding. The algorithm is differentiable by using a soft-gating approach, which approximates discrete candidate selection by a probabilistic mixture of the constituents available in a given cell of the chart. While their work relies on annotated downstream tasks to learn structures,\cite{dblp:conf/naacl/drozdovvyim19} propose a novel auto-encoder-like pretraining objective based on the inside-outside algorithm~\cite{Baker1979TrainableGF,DBLP:conf/icgi/Casacuberta94} but is still of cubic complexity. To tackle the $O(n^3)$ limitation of CKY encoding, \cite{hu-etal-2021-r2d2} propose an MLM-like pretraining objective and a pruning strategy, which reduces the complexity of encoding to linear and makes the model possible to pretrain on large-scale corpora.
\vspace{-5pt}
\paragraph{Multi-Instance Learning.}
Multi-Instance learning (MIL) deals with problems where labels are associated with groups of instances or bags (spans in our case), while instance labels are unobserved. The goal is either to label bags~\cite{DBLP:conf/nips/KeelerRL90,DBLP:journals/ai/DietterichLL97,DBLP:conf/icml/MaronR98} or to simultaneously infer bag and instance labels~\cite{DBLP:conf/icml/ZhouSL09,DBLP:conf/kdd/KotziasDFS15}. \cite{DBLP:journals/tacl/AngelidisL18} apply MIL to segment-level sentiment analysis based on an attention-based scoring method. In our work, we refine instances to different semantic granularities and consider hierarchical relationships between instances.
\vspace{-5pt}
\paragraph{Model Interpretability.} In the line of work on model interpretability, many approaches have been proposed. ~\cite{ribeiro-etal-2016-trust,DBLP:conf/nips/LundbergL17} try to generate explanation for prediction. ~\cite{DBLP:journals/jmlr/BaehrensSHKHM10,DBLP:journals/corr/SimonyanVZ13,DBLP:conf/icml/SundararajanTY17} analyze attribution by gradients. The above-mentioned methods are all posthoc. ~\cite{DBLP:conf/emnlp/KimYKY20,DBLP:conf/emnlp/CaoSAT20, DBLP:conf/emnlp/ChenJ20} apply masks on the model input in text classification to obtain token weights, but single-dimensional weights are not enough to reflect multi-label interpretation. ~\cite{DBLP:conf/nips/Alvarez-MelisJ18,rudin2019stop} argue interpretability should be an inherent property of a deep neural network and propose corresponding model architectures. However, all the above-mentioned methods are not able to generate constituent-level interpretability.
